SPGNet: Semantic Prediction Guidance for Scene Parsing

Multi-scale context module and single-stage encoder-decoder structure are commonly employed for semantic segmentation. The multi-scale context module refers to the operations to aggregate feature responses from a large spatial extent, while the single-stage encoder-decoder structure encodes the high-level semantic information in the encoder path and recovers the boundary information in the decoder path. In contrast, multi-stage encoder-decoder networks have been widely used in human pose estimation and show superior performance than their single-stage counterpart. However, few efforts have been attempted to bring this effective design to semantic segmentation. In this work, we propose a Semantic Prediction Guidance (SPG) module which learns to re-weight the local features through the guidance from pixel-wise semantic prediction. We find that by carefully re-weighting features across stages, a two-stage encoder-decoder network coupled with our proposed SPG module can significantly outperform its one-stage counterpart with similar parameters and computations. Finally, we report experimental results on the semantic segmentation benchmark Cityscapes, in which our SPGNet attains 81.1% on the test set using only 'fine' annotations.

==> tables/cityscapes_input_size.tex <==
\begin{table}[!t]
\centering
\scalebox{1}{
\begin{tabular}{c c c}
\toprule[0.2em]
 Method  & crop size  & mIoU ($\%$) \\
\toprule[0.2em]
 Baseline & $385\times385$ &  $\textbf{72.07}$       \\
 SPG & $385\times385$&  $68.62$        \\
\midrule
 Baseline & $513\times513$ &  $\textbf{75.21}$       \\
 SPG & $513\times513$&  $74.37$        \\
\midrule
 Baseline & $769\times769$ &  $76.31$       \\
 SPG & $769\times769$&  $\textbf{77.67}$        \\
\bottomrule[0.1em]
\end{tabular}
}
\caption{Cityscapes val ablation studies on training crop size. All models use ResNet-18 in encoder. SPG requires larger training crop size.}
\label{table:cityscapes_input_size}
\end{table}
